Thermal Barrier Coatings in burner rig experiment analyzed through LAser Shock for DAmage Monitoring (LASDAM) method

This study investigates failure mechanisms in a typical thermal barrier coating (TBC) system comprising an EB-PVD columnar top coat, an aluminide bond coat, and a Ni-based single crystal superalloy substrate, simulating gas turbine operating conditions using a burner rig. TBC degradation, initiated by interfacial defects from the LASAT method, was studied during thermal gradient cycling under fast and slow cooling. In-situ optical and infrared imaging, along with ex-situ SEM cross-sectional analysis, monitored failure mechanisms. The Laser Shock for Damage Monitoring (LASDAM) technique provided insights into gradient and cooling rate impacts on columnar TBC damage. Results showed significant effects of cooling rate on delamination and localized failure at blister sites, with LASDAM revealing significant overheating at damage sites. Analysis included full-field temperature and damage assessment, emphasizing blister-driven delamination under severe thermal gradients. Discussion focused on elastic stored energy effects, noting that fast cooling induced transient conditions where reversed temperature gradients increased damage, limiting TBC lifespan

==> totodiff <==
2d1
< 
10,11d8
< \graphicspath{{figs/}}
< %\usepackage{graphicx}
17c14
< \bibliographystyle{elsarticle-num}
---
> %\bibliographystyle{elsarticle-num}
22,23c19,20
< \usepackage[xcolor=dvipsnames]{changes}
< \definechangesauthor[name=SD, color=Orange]{SD}
---
> %\usepackage[xcolor=dvipsnames]{changes}
> %\definechangesauthor[name=SD, color=Orange]{SD}
33,40d29
< %\documentclass[review,numbers,sort&compress]{elsarticle}
< %\documentclass[preprint,10pt,3p]{elsarticle}
< %\usepackage{graphicx}
< \usepackage{lineno,hyperref}
< \usepackage{version}
< \usepackage{float} 
< \usepackage{textcomp}
< \usepackage{amsmath} 
42,46d30
< \usepackage{graphicx,pslatex,float,color,array,amssymb,amsmath,euscript}
< \graphicspath{{FIG/}}
< %\usepackage{graphicx}
< \usepackage{subcaption}
< \usepackage{multirow}
48,51c32
< \usepackage{gensymb}
< \usepackage{siunitx}
< %\bibliographystyle{elsarticle-num}
< \bibliographystyle{model1a-num-names}
---
> %\bibliographystyle{model1a-num-names}
53,54d33
< \usepackage[english]{babel}
< \usepackage[utf8]{inputenc}
60c39
< \modulolinenumbers[5]
---
> %\modulolinenumbers[5]
73,74c52
< %
< \def\rev#1{\color{Blue}{#1}\color{Std}}
---
> %\def\rev#1{\color{Blue}{#1}\color{Std}}
75a54,55
> %
> \def\rev#1{\color{Std}{#1}\color{Std}}
90c70
< %% please give \usepackage{epsfig}
---
> %% please give \usepackage-eps-converted-to.pdffig}
93c73
< \usepackage{amssymb}
---
> %%\usepackage{amssymb}
155a136,137
> \rev{This study investigates failure mechanisms in a typical thermal barrier coating (TBC) system comprising an EB-PVD columnar top coat, an aluminide bond coat, and a Ni-based single crystal superalloy substrate, simulating gas turbine operating conditions using a burner rig. TBC degradation, initiated by interfacial defects from the LASAT method, was studied during thermal gradient cycling under fast and slow cooling. In-situ optical and infrared imaging, along with ex-situ SEM cross-sectional analysis, monitored failure mechanisms. The Laser Shock for Damage Monitoring (LASDAM) technique provided insights into gradient and cooling rate impacts on columnar TBC damage. Results showed significant effects of cooling rate on delamination and localized failure at blister sites, with LASDAM revealing significant overheating at damage sites. Analysis included full-field temperature and damage assessment, emphasizing blister-driven delamination under severe thermal gradients. Discussion focused on elastic stored energy effects, noting that fast cooling induced transient conditions where reversed temperature gradients increased damage, limiting TBC lifespan}.
> 
157c139
< This study aims to enhance the understanding of failure mechanisms for a typical thermal barrier coating (TBC) system, made of EB-PVD columnar top coat associated with an aluminide bond coat and Ni-based single crystal superalloy as the substrate. Thermal conditions similar to the operating thermal environment in a gas turbine are tested using a burner rig. The degradation of TBCs from initial interfacial defects introduced by the LASAT method is monitored during thermal gradient cycling for a fast cooling condition and a slow cooling condition. The respective failure mechanisms are analyzed in situ by optical and infrared imaging and ex situ by SEM cross-sectional analysis. This method, the Laser Shock for Damage Monitoring (LASDAM) technique, offers insight into the impact of gradient and cooling rate on damage rate for columnar TBC systems. The results show a significant effect of cooling rate on both delamination damage and localized failure at the blister site. LASDAM also highlights, for the first time, significant overheating at the damage site. A comprehensive analysis is proposed based on experimental full-field analysis of temperature and damage, with special attention given to blister-driven delamination in the context of severe thermal gradients. Lastly, the effects of gradient and cooling rates are discussed through the analysis of elastic stored energy in the TBC system. The fast cooling rate induces a transient situation where the temperature gradient reverses (the TBC surface cooling below the substrate temperature), directly increasing damage and limiting the lifetime of the TBC. %Finite element analysis shows that rapid cooling generates tensile stresses in the top coat. 
---
> %This study aims to enhance the understanding of failure mechanisms \rev{for a typical thermal barrier coating (TBC) system, made of EB-PVD columnar top coat associated with an aluminide bond coat and Ni-based single crystal superalloy as the substrate}. Thermal conditions similar to the operating thermal environment in a gas turbine \rev{are tested using a burner rig}. The degradation of TBCs from initial interfacial defects introduced by the LASAT method is monitored during thermal gradient cycling for a fast cooling condition and a slow cooling condition. The respective failure mechanisms are analyzed in situ by optical and infrared imaging and ex situ by SEM cross-sectional analysis. \rev{This method, the Laser Shock for Damage Monitoring (LASDAM) technique, offers insight into the impact of gradient and cooling rate on damage rate for columnar TBC systems}. The results show a significant effect of cooling rate on both delamination damage and localized failure at the blister site. \rev{LASDAM also highlights, for the first time, significant overheating at the damage site. A comprehensive analysis is proposed based on experimental full-field analysis of temperature and damage, with special attention given to blister-driven delamination in the context of severe thermal gradients. Lastly, the effects of gradient and cooling rates are discussed through the analysis of elastic stored energy in the TBC system. The fast cooling rate induces a transient situation where the temperature gradient reverses (the TBC surface cooling below the substrate temperature), directly increasing damage and limiting the lifetime of the TBC}. %Finite element analysis shows that rapid cooling generates tensile stresses in the top coat. 
175c157
< \label{sec:sample1} 
---
> \label{sec:intro} 
180c162
< These findings underscore the necessity for robust experiments to investigate blister-driven delamination thoroughly. In line with this perspective, the LAser Shock for DAmage Monitoring (LASDAM) technique introduces new avenues for analyzing the driving forces behind delamination from an initial blister subjected to thermal cycling in a furnace \cite{Mahfouz:2023}. LASDAM involves inducing an artificial decohesion at the weak interface of the Thermal Barrier Coating (TBC) and monitoring its evolution during cycling. The former is achieved through precise control of the decohesion size and location using the LAser Shock Adhesion Testing (LASAT) technique \cite{boustie:2007}. The latter entails combining in-situ high-resolution CCD images, infrared thermography (IRT), and the measurement of 3D blister morphology. When applying the LASDAM method with thermal cycling in a furnace, it was observed that a significant initial increase in blister buckling precedes further delamination \cite{guipont:2019}. The driving forces for buckling were also identified as driving forces for this blister-driven delamination, a major intrinsic failure mode in TBCs \cite{Mahfouz:2023}.
---
> These findings underscore the necessity for robust experiments to investigate blister-driven delamination thoroughly \cite{scotson2024characterisation}. In line with this perspective, the LAser Shock for DAmage Monitoring (LASDAM) technique introduces new avenues for analyzing the driving forces behind delamination from an initial blister subjected to thermal cycling in a furnace \cite{Mahfouz:2023}. LASDAM involves inducing an artificial decohesion at the weak interface of the Thermal Barrier Coating (TBC) and monitoring its evolution during cycling. The former is achieved through precise control of the decohesion size and location using the LAser Shock Adhesion Testing (LASAT) technique \cite{boustie:2007}. The latter entails combining in-situ high-resolution CCD images, infrared thermography (IRT), and the measurement of 3D blister morphology. When applying the LASDAM method with thermal cycling in a furnace, it was observed that a significant initial increase in blister buckling precedes further delamination \cite{guipont:2019}. The driving forces for buckling were also identified as driving forces for this blister-driven delamination, a major intrinsic failure mode in TBCs \cite{Mahfouz:2023}.
207,208c189,190
< 		\includegraphics[width=0.55\textwidth]{figures/plan_new.jpg}
< 	\caption {Samples geometry (dimensions are given in mm)}
---
> 		\includegraphics[width=0.55\textwidth]{plan_new.jpg}
> 	\caption {Samples geometry \rev{(dimensions are given in mm)}}
220,226d201
< %\begin{figure}[H]
< %	\centering
< %		\includegraphics[width=1.\textwidth]{figures/IR_new.jpg}
< %	\caption{LASAT blisters introduced respectively on samples PC19, PC25 and PC29, observed using infrared thermography.}
< %	\caption{LASAT blisters introduced respectively on samples PC19, PC25 and PC29, observed using infrared thermography.}
<  %\label{fig:IR}
< %\end{figure}
230c205
< Moreover, optical observations allow for the examination of whether delamination leads to buckling of the TC and if the resulting blister exhibits cracking or experiences local/total spallation. Notably, for higher laser energies, a characteristic LASAT transition from a "perfect blister" (without cracking or spallation) to a cracked/spalled state has been identified for a given TBC. This transition can be discerned by plotting a LASAT curve \cite{sapardanis:2016}. The pointed arrow in Figure \ref{fig:LASAT} emphasizes this transition, indicating the onset of spallation, with full symbols denoting perfect blisters and empty ones signifying local or total spallation. The SEM cross section of a blister from the reference sample used to plot the "LASAT curve" is shown in figure \ref{fig:SEM_LASAT}. It shows significant oxidation, oxide thickness locally reaching \SI{2}{\micro\meter}, and phase transformation from $\beta$ to $\gamma'$ phase, along with decohesion occurring at the interface between the oxide layer and the top coat layer, consistently with previous results \cite{guipont:2019}. The localization of the decohesion induced by LASAT confirms that the pre-aging weakens the oxide/top coat interface properties, consistent with the state-of-the-art for such TBC systems.
---
> Moreover, optical observations allow for the examination of whether delamination leads to buckling of the TC and if the resulting blister exhibits cracking or experiences local/total spallation. Notably, for higher laser energies, a characteristic LASAT transition from a "perfect blister" (without cracking or spallation) to a cracked/spalled state has been identified for a given TBC. This transition can be discerned by plotting a LASAT curve \cite{sapardanis:2016}. The pointed arrow in Figure \ref{fig:LASAT} emphasizes this transition, indicating the onset of spallation, with full symbols denoting perfect blisters and empty ones signifying local or total spallation. \rev{The SEM cross section of a blister from the reference sample used to plot the "LASAT curve" is shown in figure \ref{fig:SEM_LASAT}. It shows significant oxidation, oxide thickness locally reaching \SI{2}{\micro\meter}, and phase transformation from $\beta$ to $\gamma'$ phase, along with decohesion occurring at the interface between the oxide layer and the top coat layer, consistently with previous results \cite{guipont:2019}. The localization of the decohesion induced by LASAT confirms that the pre-aging weakens the oxide/top coat interface properties, consistent with the state-of-the-art for such TBC systems}.
236c211
<      \includegraphics[width=\textwidth]{figures/PC29_IR.jpg}
---
>      \includegraphics[width=\textwidth]{PC29_IR.jpg}
242c217
< 	 \includegraphics[width=\textwidth]{figures/LASAT_new.jpg}%w.eps}
---
> 	 \includegraphics[width=\textwidth]{LASAT_new-eps-converted-to.pdf}
248c223
< 	 \includegraphics[width=\textwidth]{figures/IMG_6887.jpeg}%w.eps}
---
> 	 \includegraphics[width=\textwidth]{IMG_6887.jpeg}%w-eps-converted-to.pdf}
252c227
< 	\caption{LASAT method: (a) Infrared thermography (IRT) employed for assessing the debonded diameter after laser shock   (b) Equivalent debonded diameters derived from IRT, with the arrow marking the initial occurrence of local spallation (full symbols denote perfect blisters, while empty symbols represent blisters with local or total spallation)   (c) SEM cross section of a blister from the reference sample after LASAT test}
---
> 	\caption{LASAT method: (a) Infrared thermography (IRT) employed for assessing the debonded diameter after laser shock   (b) Equivalent debonded diameters derived from IRT, with the arrow marking the initial occurrence of local spallation (full symbols denote perfect blisters, while empty symbols represent blisters with local or total spallation).}
256,262d230
< %\begin{figure}[H]
< %	\centering
< %		\includegraphics[width=0.55\textwidth]{figures/IMG_6863.jpeg}%draft car tif ne passe pas:(
< %	\caption{SEM cross-sectional image of a decohesion on the reference LASAT sample.}
< % \label{fig:SEM_LASAT0}
< %\end {figure}
< 
295c263
< 		\includegraphics[width=0.75\textwidth]{figures/burner_rig.jpg}
---
> 		\includegraphics[width=0.75\textwidth]{burner_rig.jpg}
300c268
< In this study, the temperature was set to \SI{1200}{\celsius} on the ceramic surface and \SI{1050}{\celsius} in the substrate. The coating's emissivity ($\epsilon$) was assumed to be constant at 1. While this value is considered to underestimate the surface temperature by approximately 3\%, realistic emissivity values for YSZ ceramic in the pyrometer's wavelength range are around 0.98. However, emissions from the flame within the same spectral range partially counteract the impact of an overestimated emissivity \cite{Vassen2020}. Furthermore, it's important to note that the emissivity at the blisters might vary. This variability introduces uncertainty into the measurements, which is later addressed and considered in the analysis.
---
> In this study, the temperature was set to \SI{1200}{\celsius} on the ceramic surface and \SI{1050}{\celsius} in the substrate. The coating's emissivity ($-eps-converted-to.pdfilon$) was assumed to be constant at 1. While this value is considered to underestimate the surface temperature by approximately 3\%, realistic emissivity values for YSZ ceramic in the pyrometer's wavelength range are around 0.98. However, emissions from the flame within the same spectral range partially counteract the impact of an overestimated emissivity \cite{Vassen2020}. \rev{Furthermore, it's important to note that the emissivity at the blisters might vary. This variability introduces uncertainty into the measurements, which is later addressed and considered in the analysis}.
322c290
<         \includegraphics[width=\textwidth]{figures/Cycle_baf_Julich_new.jpg}%w.eps}
---
>         \includegraphics[width=\textwidth]{Cycle_baf_Julich_new-eps-converted-to.pdf}
328c296
<         \includegraphics[width=\textwidth]{figures/Cycle_baf_Julich_DT_new.jpg}
---
>         \includegraphics[width=\textwidth]{Cycle_baf_Julich_DT_new-eps-converted-to.pdf}
342c310
<         \includegraphics[width=\textwidth]{figures/champ_thermique_slow.jpg}
---
>         \includegraphics[width=\textwidth]{champ_thermique_slow.jpg}
347c315
<         \includegraphics[width=\textwidth]{figures/champ_thermique_fast.jpg}
---
>         \includegraphics[width=\textwidth]{champ_thermique_fast.jpg}
352c320
<         \includegraphics[width=\textwidth]{figures/profilsPC29_new.jpg}
---
>         \includegraphics[width=\textwidth]{profilsPC29_new.jpg}
357c325
<         \includegraphics[width=\textwidth]{figures/profilsPC19_new.jpg}
---
>         \includegraphics[width=\textwidth]{profilsPC19_new.jpg}
367,381d334
< %\begin{figure}[H]
< %    \centering
< %    \begin{subfigure}[b]{0.45\textwidth}
< %        \centering
< %        \includegraphics[width=\textwidth]{figures/profilsPC29.jpg}
< %        \caption{BR-slow (PC29)\label{fig:Tgrad29}}
< %    \end{subfigure}
< %    \begin{subfigure}[b]{0.45\textwidth}
< %        \centering
< %        \includegraphics[width=\textwidth]{figures/profilsPC19.jpg}
< %        \caption{BR-fast (PC19) \label{fig:Tgrad19}}
< %    \end{subfigure}
< %    \caption{Temperature distribution along vertical profile line passing through blisters (a) on sample PC29 tested with slow cooling rate ; (b) on sample PC19 tested with fast coooling rate.}
<  %   \label{fig:profilsT}
< %\end{figure}
383d335
< Regardless of the maximum temperature recorded at the centers of the blisters, similar local temperatures are experienced at the edges of the blisters and their associated crack tips for both BR-fast and BR-slow conditions, approximately ranging from 1215 to $\SI{1220}{\celsius}$ at blister location #3. At blister location #2, corresponding to a lower temperature, both the local temperature and temperature gradient exhibit remarkable similarity for both conditions. These consistent observations affirm the robustness of the chosen experimental setup.
385c337,339
< The observed overheating linked to each blister is likely a result of a layer of air beneath the blister, limiting the conduction of heat to the substrate. The maximum temperature observed in the center of a blister corresponds to the location of the maximum air gap thickness, while the gradual temperature decrease toward the edges of a blister corresponds to a continuous reduction in the air gap thickness, which raises questions about the influence of the blister's local height on overheating.
---
> Regardless of the maximum temperature recorded at the centers of the blisters, similar local temperatures are experienced at the edges of the blisters and their associated crack tips for both BR-fast and BR-slow conditions, approximately ranging from 1215 to $\SI{1220}{\celsius}$ at blister location \#3. At blister location \#2, corresponding to a lower temperature, both the local temperature and temperature gradient exhibit remarkable similarity for both conditions. These consistent observations affirm the robustness of the chosen experimental setup.
> 
> The observed overheating linked to each blister is likely a result of a layer of air beneath the blister, limiting the conduction of heat to the substrate. The maximum temperature observed in the center of a blister corresponds to the location of the maximum air gap thickness, while the gradual temperature decrease toward the edges of a blister corresponds to a continuous reduction in the air gap thickness, \rev{which raises questions about the influence of the blister's local height on overheating.}
398d351
< % \includegraphics[width=0.7\textwidth]{figures/T_cloques_PC29.jpg}
401c354
<         \includegraphics[width=\textwidth]{figures/T_cloques_PC29_new.jpg}
---
>         \includegraphics[width=\textwidth]{T_cloques_PC29_new-eps-converted-to.pdf}
406c359
<         \includegraphics[width=\textwidth]{figures/T_cloques_PC19_new.jpg}
---
>         \includegraphics[width=\textwidth]{T_cloques_PC19_new-eps-converted-to.pdf}
419,420d371
< %This inversion of temperature gradient has implications on the stress sign in the coating during cooling and will be discussed later. 
< 
425c376
<         \includegraphics[width=\textwidth]{figures/cooling_PC29_N=500_new.jpg}
---
>         \includegraphics[width=\textwidth]{cooling_PC29_N=500_new-eps-converted-to.pdf}
430c381
<         \includegraphics[width=\textwidth]{figures/cooling_PC19_N=90_new.jpg}
---
>         \includegraphics[width=\textwidth]{cooling_PC19_N=90_new-eps-converted-to.pdf}
447c398
< 		\includegraphics[width=0.95\textwidth]{figures/PC29.jpg}
---
> 		\includegraphics[width=0.95\textwidth]{PC29.jpg}
459c410
<         \includegraphics[width=\textwidth]{figures/Image2.jpg}
---
>         \includegraphics[width=\textwidth]{Image2.jpg}
464c415
<         \includegraphics[width=\textwidth]{figures/Image1.jpg}
---
>         \includegraphics[width=\textwidth]{Image1.jpg}
473,474d423
< %Local temperatures measured at the center of the blisters with infrared thermography at cycle 250 during cooling  show a significant temperature increase for blisters PC19-1 and PC19-3, reaching extreme temperatures of about 1600 Â°C. Cooling through the substrate is significantly inhibited as blistering and cracking occur. The local maximum temperature for blister PC19-2 has increased to about 1300Â°C, and the average temperature in the central adhesive area of the top coat is fairly unchanged at about 1230Â°C. The cycle was stopped at N=320.
< 
478c427
< 		\includegraphics[width=0.95\textwidth]{figures/PC19.jpg}
---
> 		\includegraphics[width=0.95\textwidth]{PC19.jpg}
489d437
< %This point should be related to the fact that exposure time to the highest temperature is longer than for BR-fast cycle (due to the delay in spallation event for BR-slow condition).
494,496c442,443
< 		%\includegraphics[width=0.95\textwidth]{figures/surfaceSEMPC25.jpeg}
< 		\includegraphics[width=0.95\textwidth]{figures/microIRTB_PC25.png}%PC25detailcomp3.jpeg}
< 	\caption{Ex situ analysis of a sample tested with BR-slow cooling rate (sample B): (a) IRT observation of the surface of the specimen, (b) SEM surface observation of location B-2 orange dashed line corresponds to initial location of debonding processed by LASAT, orange arrows indicate further decohesion under burner rig cycling, (c) SEM surface observation of location B-3 and (d) SEM cross-section corresponding to the black dot lines in (a) and (b) at the location B-2. }
---
> 		\includegraphics[width=0.95\textwidth]{microIRTB_PC25.png}%PC25detailcomp3.jpeg}
> 	\caption{Ex situ analysis of a sample tested with BR-\rev{slow } cooling rate (sample B): \rev{(a) IRT observation of the surface of the specimen, (b) SEM surface observation of location B-2 orange dashed line corresponds to initial location of debonding processed by LASAT, orange arrows indicate further decohesion under burner rig cycling, (c) SEM surface observation of location B-3 and (d) SEM cross-section corresponding to the black dot lines in (a) and (b) at the location B-2. }}
501c448,450
< The global surface view shown in Figure \ref{fig:PC25ex}(b), corresponding to blister B-2, shows the initial debonding site processed by LASAT, highlighted by the dashed line. The maximum observed wrinkling is confined within a circular region, clearly showing the onset of debonding. Beyond this region of initial debonding, one can observe the area where the interfacial crack has grown from this initial debonding site in the direction of the arrows, and in this area, few local undulations are observed, consistent with established findings that rumpling manifests exclusively at points of local decohesion \cite{Mahfouz:2023}. Similarly, cross-sectional analysis of bubble B-2, as shown in Figure \ref{fig:PC25ex}(d), confirms that the peak of rumpling occurs beneath the blister and is significantly reduced in regions where the topcoat adheres to the substrate. In addition, the adherent portion of the topcoat layer shows no signs of sintering, consistent with the lower surface temperature measured in this particular area, see Figure \ref{fig:Tgrad29}.    
---
> The global surface view shown in Figure \ref{fig:PC25ex}(b), corresponding to blister B-2, shows the initial debonding site processed by LASAT, \rev{highlighted by the dashed line}. The maximum observed rumpling is confined within a circular region, clearly showing the onset of debonding. Beyond this region, \rev{one can observe the area where the interfacial crack has grown from this initial debonding site in the direction of the arrows. In this area of further debonding, } few local undulations are observed, consistent with established findings that rumpling manifests exclusively at points of local decohesion \cite{Mahfouz:2023}. Similarly, cross-sectional analysis of blister B-2, as shown in Figure \ref{fig:PC25ex}(d), confirms that the peak of rumpling occurs beneath the blister and is significantly reduced in regions where the topcoat adheres to the substrate. In addition, the adherent portion of the topcoat layer shows no signs of sintering, consistent with the lower surface temperature measured in this particular area, \rev{see Figure \ref{fig:Tgrad29}}.    
> 
>     
510c459
< 	\caption{Ex situ analysis of a sample tested with BR-fast cooling rate (sample C): (a) IRT observation of the surface of the specimen, with detail of location C-1 (b) SEM surface observation of location C-2 and C-4, (c) SEM surface observation of location C-3 and (d) SEM cross-section corresponding to the black dot line in (a) at the location C-1. }
---
> 	\caption{Ex situ analysis of a sample tested with BR-fast cooling rate (sample C): \rev{(a) IRT observation of the surface of the specimen, (b) SEM surface observation of location B-2 orange dashed line corresponds to initial location of debonding processed by LASAT, orange arrows indicate further decohesion under burner rig cycling, (c) SEM surface observation of location B-3 and (d) SEM cross-section corresponding to the black dot lines in (a) and (b) at the location B-2. }}
514,531d462
< %\begin{figure}[H]
< %	\centering
< %		\includegraphics[width=0.95\textwidth]{figures/PC19details1.jpeg}
< %	\caption{Ex situ surface analysis of a sample tested with BR-fast cooling rate (specimen \# PC19).}
<  % \label{fig:PC19ex}
< %\end{figure}
< 
< 
< The cross-sectional analysis along the line connecting blisters C-1 and C-2 in Figure \ref{fig:PC19exc}(a) reveals a noteworthy correlation between local high temperature during cycling and the sintering process, as depicted in Figure \ref{fig:PC19exc}(d). At the center of blister C-1, a highly dense microstructure is evident, indicative of localized extremely high temperatures. Importantly, the sintering is more pronounced in the lower part of the top coat (TC) throughout its thickness, consistent with local compressive stresses induced by the bending of the ceramic layer, but also corresponding to an initial denser part of the ceramic layer.
< 
< Remarkably, at the location of the crack tip, and consistent with the lower local temperature, no discernible evidence of sintering is observed, as illustrated in Figure fig:PC19exc(d). This observation underscores that, despite the elevated local temperature resulting from the blister-induced air gap, the crack propagates in an area characterized by lower and more uniform temperatures within the specimen's region of interest. In essence, the hot points induced by the air gap solely influence the temperature of the blisters, and blister driven delamination is analyzed at the targeted temperature.
< 
< %\begin{figure}[H]
< %	\centering
< %		\includegraphics[width=0.95\textwidth]{figures/PC19CS1.jpeg}
< %	\caption{Ex situ cross-section analysis of a sample tested with BR-fast cooling rate (specimen \# PC19), corresponding to blister \#1 in Figure \ref{fig:PC19ex}.}
<  % \label{fig:PC19cs}
< %\end{figure}
532a464,466
> The cross-sectional analysis along the line connecting blisters C-1 and C-2 in Figure \ref{fig:PC19exc}(a) reveals a noteworthy correlation between local high temperature during cycling and the sintering process, as depicted in Figure \ref{fig:PC19exc}(d). At the center of blister C-1, a highly dense microstructure is evident, indicative of localized extremely high temperatures. Importantly, the sintering is more pronounced in the lower part of the top coat (TC) throughout its thickness, consistent with local compressive stresses induced by the bending of the ceramic layer, \rev{but also corresponding to an initial denser part of the ceramic layer}.
> 
> Remarkably, at the location of the crack tip, and consistent with the lower local temperature, no discernible evidence of sintering is observed, as illustrated in Figure \ref{fig:PC19exc}(d). This observation underscores that, despite the elevated local temperature resulting from the blister-induced air gap, the crack propagates in an area characterized by lower and more uniform temperatures within the specimen's region of interest. In essence, the hot points induced by the air gap solely influence the temperature of the blisters, and blister driven delamination is analyzed at the targeted temperature.
537d470
< %Lastly, it is essential to acknowledge that, given the data's reliance on cross-sectional image analysis and considering the inherent variability observed in the EB-PVD deposition process, the initial porosity may vary from one sample to another.
540,546d472
< %143 microns
< %\begin{figure}[H]
< %	\centering
< %		\includegraphics[width=0.95\textwidth]{figures/poros1_40pxgl10_1.jpg}
< %	\caption{Porosity as a function of the distance to the center of the blister r}
< %  \label{fig:porosity}
< %\end{figure}
550c476
<    \includegraphics[width=0.95\textwidth]{figures/IMG_6843.jpeg}%poros1_40pxgl10_2_new.eps}
---
>    \includegraphics[width=0.95\textwidth]{poros1_40pxgl10_2_new-eps-converted-to.pdf} %IMG_6843.jpeg}%
557c483
<         \includegraphics[width=\textwidth]{figures/eox.jpg}%.eps}  
---
>         \includegraphics[width=\textwidth]{eox-eps-converted-to.pdf}  
562c488
<         \includegraphics[width=\textwidth]{figures/fs.jpg}%.eps}
---
>         \includegraphics[width=\textwidth]{fs-eps-converted-to.pdf}
568c494
<     \caption{Microstructure evolution represented by oxide and phase tranformation : BR (current study) vs and S-FCT (data from \cite{soulignac2014prevision})}
---
>     \caption{Microstructure \rev{analysis considering (a) variation of porosity as a function of the distance from the center of the blister, (b) oxide thickness and (c) $\gamma$' phase fraction } evolutions for burner rig (BR/current study) and furnace cycling (S-FCT/data from \cite{soulignac2014prevision})}
573c499
< In addition to sintering of the top coat, SEM cross sections allow assessment of both local oxide thickness and phase transformation in the bond coat layer, from $\beta$-NiAl to $\gamma$'-Ni$_3$Al, Figures \ref{fig:evolutionmic}(b) and (c), respectively. Both were measured using SEM observations and segmentation through standard thresholding techniques using ImageJ/Fiji software \cite{ImageJ:2024}, for regions approximately \SI{1.4}{mm} wide in adherent top coat areas. The $\gamma'$ phase fraction corresponds to the surface fraction of the outer layer, defined as the area between the oxide layer and the embedded grit alumina particles, see Figure \ref{fig:SEM_LASAT}.
---
> In addition to sintering of the top coat, SEM cross sections allow assessment of both local oxide thickness and phase transformation in the bond coat layer, from $\beta$-NiAl to $\gamma$'-Ni$_3$Al, Figures \ref{fig:evolutionmic}(b) and (c), respectively. \rev{Both were measured using SEM observations and segmentation through standard thresholding techniques using ImageJ/Fiji software \cite{ImageJ:2024}, for regions approximately \SI{1.4}{mm} wide in adherent top coat areas. The $\gamma'$ phase fraction corresponds to the surface fraction of the outer layer, defined as the area between the oxide layer and the embedded grit alumina particles, see Figure \ref{fig:SEM_LASAT}}.
581c507
< %The crack tip (bottom of the blister) corresponds to a slight modification of temperature. Thus, damage triggered by local maxima of temperature should be seen on the one hand, as a factor damaging locally the blister itself. On the other hand, local maxima of temperature could modify the loading seen by the crack tip.
---
> 
585c511
< As outlined earlier, the LASDAM technique enables the monitoring of both in situ interfacial debonding and ex situ blistering \cite{Mahfouz:2023}. The evolution of decohesion diameter as a function of the number of cycles for BR-slow testing (A and B samples) is presented in Figures \ref{fig:DPC29} and \ref{fig:DPC25}. The progression of blisters in locations 2 and 3 exhibits remarkable similarity for both specimens, particularly concerning the number of cycles leading to the initiation of debonding, which occurs around 260 cycles for both specimens: The disparity between samples A and B is minimal, with a difference of no more than 10 cycles for location 3,  as illustrated in Figure \ref{fig:blisterm_slow}. Additionally, at N=500, no debonding is observed for blister #1 in both samples. The number of debonding and spallation cycles for each blister is detailed in Table \ref{tab:specimendetails}.
---
> As outlined earlier, the LASDAM technique enables the monitoring of both in situ interfacial debonding and ex situ blistering \cite{Mahfouz:2023}. The evolution of decohesion diameter as a function of the number of cycles for BR-slow testing (A and B samples) is presented in Figures \ref{fig:DPC29} and \ref{fig:DPC25}. The progression of blisters in locations 2 and 3 exhibits remarkable similarity for both specimens, particularly concerning the number of cycles leading to the initiation of debonding, which occurs around 260 cycles for both specimens: The disparity between samples A and B is minimal, with a difference of no more than 10 cycles for location 3,  as illustrated in Figure \ref{fig:blisterm_slow}. Additionally, at N=500, no debonding is observed for blister \#1 in both samples. \rev{The number of debonding and spallation cycles for each blister is detailed in Table \ref{tab:specimendetails}}.
592,593c518,519
<         \includegraphics[width=\textwidth]{figures/D_PC29_new.jpg}%w.eps}
<         \caption{Debonded diameter sample A \label{fig:DPC29}}
---
>         \includegraphics[width=\textwidth]{D_PC29_new-eps-converted-to.pdf}
>         \caption{Debonded diameter \rev{sample A} \label{fig:DPC29}}
597,598c523,524
<         \includegraphics[width=\textwidth]{figures/D_PC25_new.jpg}%w.eps}
<         \caption{Debonded diameter  sample B \label{fig:DPC25}}
---
>         \includegraphics[width=\textwidth]{D_PC25_new-eps-converted-to.pdf}
>         \caption{Debonded diameter  \rev{sample B} \label{fig:DPC25}}
602,603c528,529
<    		\includegraphics[width=\textwidth]{figures/delta_PC29_new.jpg}%w.eps}
< 	\caption{Blisters height sample A}
---
>    		\includegraphics[width=\textwidth]{delta_PC29_new-eps-converted-to.pdf}
> 	\caption{Blisters height \rev{sample A} }
608,609c534,535
<    		\includegraphics[width=\textwidth]{figures/T_delta.jpg}%w.eps}
< 	\caption{Maximum temperature sample A}
---
>    		\includegraphics[width=\textwidth]{T_delta-eps-converted-to.pdf}
> 	\caption{\rev{Maximum temperature sample A}}
613c539
<    Evolution of blisters under slow coooling rate: debonded diameter for samples (a) A and (b) B, and (c) blister height for sample A (full symbols denote perfect blisters, while empty symbols represent blisters with local or total spallation). (d) Evolution of maximum temperature at blisters as a function of blister height.
---
>    Evolution of blisters under slow coooling rate: debonded diameter for  (a) sample A as a function of N and (b) sample B as a function of N,  (c) blister height for sample A as function of N  \rev{and (d)   maximum temperature at blisters from sample A as a function of blister height.} (full symbols denote perfect blisters, while empty symbols represent blisters with local or total spallation)
618,620c544
< %Within 10 cycles, debonded diameter evolution plots show similar evolution for respective interface defects on both samples. 
< 
< For sample A, profilometer measurements were conducted every 100 cycles, necessitating testing interruptions. Given the analogous debonding behavior observed in both samples, these interruptions are presumed to have a minimal impact on the overall damage rate. The evolution of blister height over the number of cycles for sample A is shown in Figure \ref{fig:delta_PC29}. The results indicate that, while the equivalent delaminated diameter initially remains relatively constant, the blister height undergoes a significant increase. This trend aligns with observations made during furnace thermal cycling, where blister evolution is initially characterized by the activation of a buckling mechanism until a point is reached where further growth of interfacial debonding is observed \cite{guipont:2019}. The height evolution presented in Figure \ref{fig:delta_PC29} also illustrates a threshold, approximately \SI{50}{\micro\meter}, beyond which spallation occurs. Additionally, Figure \ref{fig:T_delta} demonstrates a consistent increase in maximum temperature, plotted previously in Figure \ref{fig:T_cloques}, with increasing blister height, supporting the importance of analyzing local overheating in understanding blister evolution.
---
> For sample A, profilometer measurements were conducted every 100 cycles, necessitating testing interruptions. Given the analogous debonding behavior observed in both samples, these interruptions are presumed to have a minimal impact on the overall damage rate. The evolution of blister height over the number of cycles for sample A is shown in Figure \ref{fig:delta_PC29}. The results indicate that, while the equivalent delaminated diameter initially remains relatively constant, the blister height undergoes a significant increase. This trend aligns with observations made during furnace thermal cycling, where blister evolution is initially characterized by the activation of a buckling mechanism until a point is reached where further growth of interfacial debonding is observed \cite{guipont:2019}. The height evolution presented in Figure \ref{fig:delta_PC29} also illustrates a threshold, approximately \SI{50}{\micro\meter}, beyond which spallation occurs. \rev{Additionally, Figure \ref{fig:T_delta} demonstrates a consistent increase in maximum temperature, plotted previously in Figure \ref{fig:T_cloques}, with increasing blister height, supporting the importance of analyzing local overheating in understanding blister evolution}.
622,628d545
< %\begin{figure}[H]
< 	%\centering
< 		%\includegraphics[width=0.45\textwidth]{figures/delta_PC29_new.jpg}
< 	%\caption{Blisters height evolution on sample PC29.}
<  % \label{fig:delta_PC29}
< %\end{figure}
< %TBD graphe en fonction du tHT et superposition avec rÃ©sultats MÃ©lanie, pour $\delta D$ et remplacer Fig 18 par $\delta h$
640,644d556
< %d_N$ and blistering $h_N$ are used for comparison purposes as:
< %\begin{equation}  d_N= \frac{D(N)-D(0)}{D(0)}\end{equation}
< %and
< %\begin{equation}h_N=\frac{\delta(N)-\delta(0)}{\delta(0)}\end{equation}
< %where D(N) and D(0) correspond to current and initial debonded diameter, and $\delta$(N) and $\delta$(0) correspond to current and initial blister height respectively.
646,647c558
< Significantly accelerated macroscopic evolution kinetics are evident for both delamination and blistering in BR fast cycling compared to BR slow cycling, as shown in Figures \ref{fig:evolutionDam}(a) and (b), respectively. To clarify the role of thermal gradient on damage rate, S-FCT data were added to these plots, combining data from four different samples.  For three of these samples, three individual blisters are examined, while one other sample contains only one blister. To emphasize the blister condition, full symbols indicate blisters with no evidence of topcoat damage, while empty symbols indicate local cracking and/or spalling of the topcoat at the blister location. In particular, local cracking or spallation manifests much earlier at the fast cooling rate, with the first local crack observed after only 10 thermal cycles and the second after 90 cycles, see Figure \ref{fig:evolutionDam} and Table \ref{tab:specimendetails} for values. In contrast, these events occur at later stages, specifically after 300 and 500 cycles, respectively, for the slow cooling rate.
< %This should have a significant impact on blistering. %It is worth noting that, despite some differences from test to test, the differences associated with blister \#3 exceed the systematic difference from PC29 to PC25.
---
> Significantly accelerated macroscopic evolution kinetics are evident for both delamination and blistering in BR fast cycling compared to BR slow cycling, as shown in Figures \ref{fig:evolutionDam}(a) and (b), respectively. \rev{To clarify the role of thermal gradient on damage rate, S-FCT data were added to these plots, combining data from four different samples.  For three of these samples, three individual blisters are examined, while one other sample contains only one blister. To emphasize the blister condition, full symbols indicate blisters with no evidence of topcoat damage, while empty symbols indicate local cracking and/or spalling of the topcoat at the blister location}. In particular, local cracking or spallation manifests much earlier at the fast cooling rate, with the first local crack observed after only 10 thermal cycles and the second after 90 cycles, see Figure \ref{fig:evolutionDam} and Table \ref{tab:specimendetails} for values. In contrast, these events occur at later stages, specifically after 300 and 500 cycles, respectively, for the slow cooling rate.
655,656c566,567
<         \includegraphics[width=\textwidth]{figures/comparaison_new.jpg}%w.eps}  
<         %\includegraphics[width=\textwidth]{figures/relativeD_new.jpg}  
---
>         \includegraphics[width=\textwidth]{comparaison_new-eps-converted-to.pdf}  
>         %\includegraphics[width=\textwidth]{relativeD_new.jpg}  
661c572
<         \includegraphics[width=\textwidth]{figures/comparaison_delta.jpg}%a.eps}
---
>         \includegraphics[width=\textwidth]{comparaison_delta-eps-converted-to.pdf}
670d580
< %\subsection{Comparative analysis of microstructure evolution under Burner Rig and under homogeneous temperature}
672,673d581
< %Because of the microstructure and temperature observations described above, the question of interfacial temperature is of course essential to compare these burner rig results with furnace cycling tests (FCT) without gradient. 
< 
679,680c587
< %Considering a similar cumulative time spent at maximum temperature, $t_{\textrm{HT}}$, the BR experiment results in a slight increase in TGO thickness, Figure \ref{fig:eoxl}.  It is plausible that the local temperature for LASDAM conducted in the burner rig facility may have exceeded \SI{1100}{\celsius}. Similarly, in terms of phase transformation, the burner rig measurements exhibit a higher $\gamma$' phase fraction compared to FCT. It is worth noting that harsh loading conditions, particularly thermomechanical fatigue (TMF) loading, are known to cause significant oxide damage (local failure), leading to a subsequent significant increase in oxide thickness \cite{Bartsch:2008}. Similarly, the phase transformation in (Ni,Pt)Al diffusion coatings is highly sensitive to TMF conditions: the higher the stress level at high temperature, the higher the rate of phase transformation from $\beta$ to $\gamma'$ \cite{Sallot:2015}. In burner rig cycling, where the cooling rate is higher than in S-FCT, the likelihood of subsequent oxide spallation and an increase in phase transformation is greater.
< Considering a similar cumulative time spent at maximum temperature, $t_{\textrm{HT}}$, the results of the BR experiment are very similar to those of the FCT regarding  oxide thickness, with the variation being relatively small compared to the inherent uncertainty in their quantification. However, the difference for phase transformation is more significant, suggesting a local lower temperature in the bond coat for burner rig compared to FCT. However, this point should be mitigated by the fact that this measurement is highly sensitive to the width of the analyzed area, e.g. as shown in previous results dealing with the same TBC system \ref{Maurel:2012f}. This suggests that the observed increase in blister evolution, both in height and debonding, is mainly controlled by a change in mechanical loading rather than a change in interfacial oxidation. The only significant difference in the microstructure evolution when comparing BR to FCT is the modification of the sintering at the center of the blister. This suggests, a priori, only a mechanical effect.
---
> \rev{Considering a similar cumulative time spent at maximum temperature, $t_{\textrm{HT}}$, the results of the BR experiment are very similar to those of the FCT regarding  oxide thickness, with the variation being relatively small compared to the inherent uncertainty in their quantification. However, the difference for phase transformation is more significant, suggesting a local lower temperature in the bond coat for burner rig compared to FCT. However, this point should be mitigated by the fact that this measurement is highly sensitive to the width of the analyzed area, e.g. as shown in previous results dealing with the same TBC system \cite{Maurel:2012f}. This suggests that the observed increase in blister evolution, both in height and debonding, is mainly controlled by a change in mechanical loading rather than a change in interfacial oxidation. The only significant difference in the microstructure evolution when comparing BR to FCT is the modification of the sintering at the center of the blister. This suggests, a priori, only a mechanical effect}.
682c589
< A robust analysis of the temperature gradient is needed to more accurately assess the temperature reached at the crack tip during the BR cycle, by the way, the microstructure was observed only on the remaining adherent areas to avoid artifacts induced by local oxide spallation. This will be addressed in a future work.
---
> \rev{A robust analysis of the temperature gradient is needed to more accurately assess the temperature reached at the crack tip during the BR cycle, by the way, the microstructure was observed only on the remaining adherent areas to avoid artifacts induced by local oxide spallation. This will be addressed in a future work}.
687,689c594
< %For the given system, previous results have been established considering homogeneous temperature through short and long duration of furnace cycling tests (FCT), with dwell times of 5 and 50 minutes respectively \cite{maurel:2019,Mahfouz:2023}.
< 
<  In a previous study on the TBC system investigated in this paper, LASDAM results were obtained under homogeneous temperature conditions throughout the system, using short Furnace Cycling Tests (FCT) with dwell times of 5 minutes \cite{Mahfouz:2023}. The same experimental methodology was then used: the interfacial defects were induced after an initial aging of 100 long FCTs (L-FCT) with a dwell time of 50 minutes at high temperature. Figures \ref{fig:drel} and \ref{fig:hrel} illustrate that both the damage rate associated with relative variations in debonded diameter and the stress buildup associated with relative variations in blister height are higher for burner rig (BR) cycling compared to S-FCT.
---
>  In a previous study on the TBC system investigated in this paper, LASDAM results were obtained under homogeneous temperature conditions throughout the system, using short Furnace Cycling Tests (FCT) with dwell times of 5 minutes \cite{Mahfouz:2023}. The same experimental methodology was then used: the interfacial defects were induced after an initial aging of 100 long FCTs (L-FCT) with a dwell time of 50 minutes at high temperature. Figures \ref{fig:drel} and \ref{fig:hrel} illustrate that \rev{both the damage rate associated with relative variations in debonded diameter and the stress buildup associated with relative variations in blister height are higher for burner rig (BR) cycling compared to S-FCT}.
691d595
<   %First comparison is addressed considering only S-FCT compared to BR experiments for same procedure: 
693,694c597,598
< Another aspect of the analysis is to evaluate the height-diameter relationship, which serves as an indicator of the stress state within the blister. In this context, for a given diameter, a higher blister height corresponds to increased stresses within the blister \cite{mcdonald:2010,Mahfouz:2023}. In the as-received (AR) condition, corresponding to the LASAT defect introduced after 100 preliminary L-FCTs, indicated by the black symbols in Figure \ref{fig:comparison}, the maximum height is approximately \SI{40}{\micro}m for a diameter of \SI{4}{mm}. No noticeable difference in height compared to the AR state is observed after 160 cycles of BR fast cycling. However, for a higher number of cycles, a trend becomes apparent indicating increased stress in the system for both BR-fast and BR-slow conditions.
< The blister height obtained under BR conditions approaches that achieved after 2015 S-FCT cycles, as indicated by the green triangle symbols in Figure \ref{fig:comparison}. This further demonstrates that BR testing is more detrimental than S-FCT, as the stress build-up is higher in the former than in the latter, in consideration of the lower number of cycles.
---
> Another aspect of the analysis is to evaluate the height-diameter relationship, which serves as an indicator of the stress state within the blister. In this context, for a given diameter, a higher blister height corresponds to increased stresses within the blister \cite{mcdonald:2010,Mahfouz:2023}. In the as-received (AR) condition, corresponding to the LASAT defect introduced after 100 preliminary L-FCTs, indicated by the black symbols in Figure \ref{fig:comparison}, the maximum height is approximately \SI{40}{\micro\meter} for a diameter of \SI{4}{mm}. No noticeable difference in height compared to the AR state is observed after 160 cycles of BR fast cycling. However, for a higher number of cycles, a trend becomes apparent indicating increased stress in the system for both BR-fast and BR-slow conditions.
> The blister height obtained under BR conditions approaches that achieved after 2015 S-FCT cycles, as indicated by the green triangle symbols in Figure \ref{fig:comparison}. This further demonstrates that BR testing is more detrimental than S-FCT, as the stress build-up is higher in the former than in the latter, \rev{in consideration of the lower number of cycles}.
700c604
<  \includegraphics[width=0.55\textwidth]{figures/dam2hbrfct.jpg}%t.eps}
---
>  \includegraphics[width=0.55\textwidth]{dam2hbrfct-eps-converted-to.pdf}
705d608
< %However, considering the microstructure analysis presented earlier, it is crucial to acknowledge that the local temperature in BR experiments might have slightly surpassed the oxidation temperature prescribed in FCT experiments. Consequently, the detrimental effect observed in the BR setup could be attributed to the higher maximum temperature at the interface.
707c610
< On the other hand, considering the similar oxidation and phase transformation rates in BR and FCT conditions, it could be assumed that the average bond coat temperature at the crack tip was similar for both test conditions. This point is of high interest because it has been shown in the LASDAM experiment that the BC plasticity plays a key role in determining the applied torque to the blister \cite{Mahfouz:2023}: the higher the plasticity in the BC, the higher the blistering and damage rate. Thus, the local behavior of the BC might be comparable.  
---
> \rev{On the other hand, considering the similar oxidation and phase transformation rates in BR and FCT conditions, it could be assumed that the average bond coat temperature at the crack tip was similar for both test conditions. This point is of high interest because it has been shown in the LASDAM experiment that the BC plasticity plays a key role in determining the applied torque to the blister \cite{Mahfouz:2023}: the higher the plasticity in the BC, the higher the blistering and damage rate. Thus, the local behavior of the BC might be comparable}.  
709d611
< %Moreover, the cooling rate in the FCT experiment is lower than that in the BR-slow condition. Consequently, the considered FCT condition is less damaging in terms of both maximum interface temperature and cooling rate parameters. %Additional tests with higher FCT temperatures are required to draw a conclusive assessment on these aspects.
711,735d612
< %\subsection{In plane gradient}
< %Final point addressed here is the heterogeneous response of blisters relative to surface temperature distribution on the ceramic surface exposed to the burner flame.
< %As already mentioned, infrared thermography acquisitions shown in Figure \ref{fig:champsT}, during high temperature dwell, highlight an eccentricity of the flame, hence a difference in thermal loading seen by each of the blisters. 
< %On sample PC19, blisters PC19-1 and and PC19-3 located in the hotter upper surface of the sample show early macroscopic damage. For slow cooling rate cycling, we observe on samples PC25 and PC29 that positions 3 and 2 are most critical. We reported in Table \ref{tab:maxT_DT}, values of maximum temperatures on each of the blisters and temperature difference values calculated on delamination front along profiles lines shown in Figure \ref{fig:profilsT}. Results suggest that damage is fastest on the blister where the temperature is highest (but temperature difference is zero or in-plane gradient is negligible on adherent top coat), followed by the blister where the in-plane gradient is the highest but the temperature is intermediate.
< 
< %\begin{table}[h]
< %    \caption{Measurements of maximum temperatures and in-plane gradients on blisters in samples PC25 and PC29 cycled with slow cooling rate.}
<  %   \centering
<   %   \begin{tabular}{c ccc ccc}
<    %  \hline
<     %     Condition&Blister&T$_{\max}$ ({\celsius})&$\Delta$T ({\celsius}) & N$_{DI}$ & N$_{crack}$ & N$_{spall}$ \\\hline
<      %    \multirow{6}{*}{BR-slow}&PC25-1&1240&10&&&\\
<       %   &PC25-2&1235&20&&&\\ 
<        %  &PC25-3&1255&0&&&\\
<         % \cline{2-2}
<         % &PC29-1&1250&8&&&\\
<          %&PC29-2&1240&25 &&&\\
<          %&PC29-3&1260&20&&&\\
<         %\cline{1-2}
<          %\multirow{3}{*}{BR-fast}&PC19-1&1250&8&&&\\
<          %&PC19-2&1250&8&&&\\
<          %&PC19-3&1250&8&&&\\
<     % \end{tabular}
<      %\label{tab:maxT_DT}
< %\end{table}
752c629
< %The plot in Figure \ref{fig:ERR_SFCT} shows the calculated normalized elastic energy in the coating upon cooling using measured surface and substrate temperatures in figure, for BR-fast and BR-slow conditions, which are compared to homogeneous furnace condition cycle tested in Figure \ref{fig:cycles}.
---
> The normalized energy release rate curves suggest a faster reaching of the maximum energy level of the system at higher cooling rates. The asymptotic values of the energy release rate at the minimum temperature are identical for both BR-slow and BR-fast conditions, but a significant transient difference is observed: BR-slow shows a monotonic energy increase, while BR-fast shows a peak in the first few seconds of cooling. As demonstrated in \cite{levi2012environmental}, the cooling of the coating relative to the substrate causes tensile stresses in the upper layer, resulting in peak energy release rates which may exceed those observed in the cooled state. This tensile stress phenomenon was further validated by finite element modeling of thermal gradient cycling in \cite{Mahfouz:2023}. Surprisingly, S-FCT achieves a higher steady-state energy than the burner rig conditions, contradicting the experimental results. \rev{The model proposed by Levi et al. \cite{levi2012environmental} explains that the energy release rate in coatings subjected to thermal cycling is influenced by two main factors: the differential contraction arising from the mismatch in thermal expansion coefficients between the substrate and the coating, and the self-constriction of the coating due to cooling at its surface. In scenarios where the cooling rate is slow for thermal gradient cycling conditions, the gradient’s effect can help alleviate the strains and stresses experienced by the coating, potentially lowering the energy release rate}. This inconsistency with experimental results suggests a potential sensitivity of damage to cooling rates, implying that faster energy input may result in greater damage. 
754d630
< The normalized energy release rate curves suggest a faster reaching of the maximum energy level of the system at higher cooling rates. The asymptotic values of the energy release rate at the minimum temperature are identical for both BR-slow and BR-fast conditions, but a significant transient difference is observed: BR-slow shows a monotonic energy increase, while BR-fast shows a peak in the first few seconds of cooling. As demonstrated in \cite{levi2012environmental}, the cooling of the coating relative to the substrate causes tensile stresses in the upper layer, resulting in peak energy release rates which may exceed those observed in the cooled state. This tensile stress phenomenon was further validated by finite element modeling of thermal gradient cycling in \cite{Mahfouz:2023}. Surprisingly, S-FCT achieves a higher steady-state energy than the burner rig conditions, contradicting the experimental results. The model proposed by Levi et al. \cite{levi2012environmental} explains that the energy release rate in coatings subjected to thermal cycling is influenced by two main factors: the differential contraction arising from the mismatch in thermal expansion coefficients between the substrate and the coating, and the self-constriction of the coating due to cooling at its surface. In scenarios where the cooling rate is slow for thermal gradient cycling conditions, the gradient’s effect can help alleviate the strains and stresses experienced by the coating, potentially lowering the energy release rate. This inconsistency with experimental results suggests a potential sensitivity of damage to cooling rates, implying that faster energy input may result in greater damage. %Despite this, when calculating the elastic energy for BR-slow and BR-fast, we assumed the interface temperature to be equal to the measured substrate temperature. %However, by considering a temperature drop of \SI{100}{\celsius} in the top coat layer, corresponding to an interface temperature of \SI{1100}{\celsius}, Figure \ref{fig:ERR_Levi} illustrates that higher elastic energy values can be achieved (indicated by the dotted line representing +\SI{50}{\celsius}).
757c633
< This model follows:
---
> \rev{This model follows:
760,761c636,637
< \end{equation}
< where $\tau$ is a parameter fitted to match the observed time to spallation, other parameters being consistent with the notations used for Levi's model in equation \ref{eq:energy}.
---
> \end{equation}}
> \rev{where $\tau$ is a parameter fitted to match the observed time to spallation, other parameters being consistent with the notations used for Levi's model in equation \ref{eq:energy}}.
767,783d642
< % Normalized energy curves show monotic increase of U with time for both BR-slow and S-FCT cycles, until steady-state uniform temperature is reached. However, unlike what was expected, maximum U is obtained for S-FCT cycle, for complete cooling to low temperature of the cycle. Normalized energy curve for BR-fast shows a peak value of energy release rate reached in the first few seconds of cooling. It is shown in \cite{levi2012environmental}, that cooling of the coating relative to the substrate develops tensile stresses in the top coat leading to peaks in energy release rates that can be higher than in the cooled state.
< 
< 
< 
< 
< %\begin{figure}[H]
< %    \centering
< %        \includegraphics[width=0.45\textwidth]{figures/U_S-FCT.jpg} 
< %   \caption{Normalized elastic energy per area in the coating calculated during cooling for BR-fast and BR-slow cycles from pyrometer and thermocouple measurements considering the initial temperature evolution and compared to S-FCT cycle. \label{fig:ERR_SFCTxxx}}
< %\end{figure}
< 
< %\begin{figure}[H]
< %   \centering
< %        \includegraphics[width=0.45\textwidth] {figures/U_T.jpg}   
<    %\caption{Evolution of normalized elastic energy per area in the coating calculated at complete cool down as a function of %$T_surf$ and for values of Tsub equal to 1050, 1100 and \SI{1150}{\celsius}}. 
<    %\label{fig:U_Txxx}
< %\end{figure}
789c648
<         \includegraphics[width=\textwidth]{figures/U_S-FCT_new.jpg}%T.eps} 
---
>         \includegraphics[width=\textwidth]{U_S-FCT_new-eps-converted-to.pdf} 
795c654
<         \includegraphics[width=\textwidth]{figures/U_S-FCT_Vassen_new.jpg}%en.eps}   
---
>         \includegraphics[width=\textwidth]{U_S-FCT_Vassen_new-eps-converted-to.pdf}   
805c664
< The thermal loading analyzed in section \ref{sec:dwell_maxT} shows that much higher temperatures were reached at the blister sites, with these local temperatures increasing during cycling as a result of blistering. Considering the temperature profiles extracted at the maximum temperatures at the blister locations from infrared thermography measurements during cooling to \SI{400}{\celsius}, normalized energy curves based on Levi's model, eq. \ref{eq:energy}, are plotted in Figure \ref{fig:U_blistersPC29} for Sample A tested with the BR slow cycle, at cycle 250 and cycle 500. This approach is a rough approximation of the mechanical state as Levi et al.'s model \cite{levi2012environmental}, subsequently used, ignores the change in stress state in the presence of a blister. The aim is to evaluate the trend in terms of the effect of overheating on the mechanical state. This analysis is subsequently only qualitative.
---
> The thermal loading analyzed in section \ref{sec:dwell_maxT} shows that much higher temperatures were reached at the blister sites, with these local temperatures increasing during cycling as a result of blistering. Considering the temperature profiles extracted at the maximum temperatures at the blister locations from infrared thermography measurements during cooling to \SI{400}{\celsius}, normalized energy curves \rev{based on Levi's model, eq. \ref{eq:energy}}, are plotted in Figure \ref{fig:U_blistersPC29} for Sample A tested with the BR slow cycle, at cycle 250 and cycle 500. This approach is a rough approximation of the mechanical state as Levi et al.'s model \cite{levi2012environmental}, subsequently used, ignores the change in stress state in the presence of a blister. The aim is to evaluate the trend in terms of the effect of overheating on the mechanical state. This analysis is subsequently only qualitative.
807c666
< Observing the cooling process at cycle 250, it is noteworthy that the elastic energy release rate calculated at the adherent top coat area exceeds that at the blister sites, Figure \ref{fig:N=250}. As explained earlier, according to Levi et al.’s model, a mild thermal gradient throughout the top coat can be beneficial and potentially lower the energy release rate. This is evident in the case of blisters A-1, A-2 and A-3 compared to the adherent top coat at N=250. However, as the gradient increases for A-2 and A-3, it amplifies the energy release rate compared to the adherent top coat. In fact, at cycle 500, the elastic energy release rate has escalated for blisters A-2 and A-3, with A-2 showing higher energy values, Figure \ref{fig:N=500}. \rev{ Figure \ref{fig:U_T} takes into account comparable maximum temperatures at the blister sites for BR-slow and BR-fast, and cooling down to 400°C, which occurs within approximately 20 seconds under fast cooling rates, and around 70 seconds under slow cooling rates. The normalized energy curves show exceptionally high energy values for blister C-3, which peaks at a normalized value of about 5.}
---
> Observing the cooling process at cycle 250, it is noteworthy that the elastic energy release rate calculated at the adherent top coat area exceeds that at the blister sites, \rev{Figure \ref{fig:N=250}}. \rev{As explained earlier, according to Levi et al.’s model, a mild thermal gradient throughout the top coat can be beneficial and potentially lower the energy release rate. This is evident in the case of blisters A-1, A-2 and A-3 compared to the adherent top coat at N=250. However, as the gradient increases for A-2 and A-3, it amplifies the energy release rate compared to the adherent top coat}. In fact, at cycle 500, the elastic energy release rate has escalated for blisters A-2 and A-3, with A-2 showing higher energy values, \rev{Figure \ref{fig:N=500}}. The normalized energy curves shown in Figure \ref{fig:U_T}, which take into account comparable maximum temperatures at the blister sites for BR-slow and BR-fast, show exceptionally high energy values for blister C-3, which peaks at a normalized value of about 5.
816c675
<         \includegraphics[width=\textwidth]{figures/N=250.jpg}%0.eps}   
---
>         \includegraphics[width=\textwidth]{N=250-eps-converted-to.pdf}   
822c681
<         \includegraphics[width=\textwidth]{figures/N=500.jpg}%0.eps}
---
>         \includegraphics[width=\textwidth]{N=500-eps-converted-to.pdf}
833c692
<  \includegraphics[width=0.55\textwidth]{figures/U_U0_blisters.jpg}%rs.eps}
---
>  \includegraphics[width=0.55\textwidth]{U_U0_blisters-eps-converted-to.pdf}
839c698
<  Local overheating of the blister dictates the steady-state behavior, highlighting the strong influence of the blister on the mechanical loading of the TBC. These results motivate numerical solutions to evaluate a more realistic mechanical state, taking into account both the temperature gradient and the mechanical evolution of the system, as well as the modification of the blister dimensions during thermal cycling. The strong correlation between local maximum temperature and blister height is a key factor in the local TBC stress as shown in Figure \ref{fig:T_delta} and should be considered in further studies. The coupling between oxidation rate, growth strain and BC creep has been established as a crucial parameter controlling the mechanical state of the TBC considering the homogeneous temperature in the FCT \cite{Mahfouz:2023}. This drastic temperature gradient should therefore play a key role in the local loading, i.e. the stress intensity factor or other driving force controlling the damage rate. 
---
>  Local overheating of the blister dictates the steady-state behavior, highlighting the strong influence of the blister on the mechanical loading of the TBC. These results motivate numerical solutions to evaluate a more realistic mechanical state, taking into account both the temperature gradient and the mechanical evolution of the system, as well as the modification of the blister dimensions during thermal cycling. \rev{The strong correlation between local maximum temperature and blister height is a key factor in the local TBC stress as shown in Figure \ref{fig:T_delta} and should be considered in further studies. The coupling between oxidation rate, growth strain and BC creep has been established as a crucial parameter controlling the mechanical state of the TBC considering the homogeneous temperature in the FCT \cite{Mahfouz:2023}. This drastic temperature gradient should therefore play a key role in the local loading, i.e. the stress intensity factor or other driving force controlling the damage rate}. 
841c700
< Last but not least, the measurement of temperature in FCT specimens is not as precise compared to the in-depth analysis of BR experiments proposed in this study: in FCT specimens, thermocouples do not take into account either the temperature gradient in the systems or the thermal inertia of the specimen, which could affect the above analysis. Furthermore, a more accurate temperature measurement should be considered for each experimental condition in order to conclude on the transient aspects in the temperature evolution and the subsequent impact on the TBC damage, this possibility being also offered by the LASDAM method.
---
> \rev{Last but not least, the measurement of temperature in FCT specimens is not as precise compared to the in-depth analysis of BR experiments proposed in this study: in FCT specimens, thermocouples do not take into account either the temperature gradient in the systems or the thermal inertia of the specimen, which could affect the above analysis. Furthermore, a more accurate temperature measurement should be considered for each experimental condition in order to conclude on the transient aspects in the temperature evolution and the subsequent impact on the TBC damage, this possibility being also offered by the LASDAM method.}
849c708
< In summary, the following findings were thoroughly addressed in this study:
---
> \rev{In summary, the following findings were thoroughly addressed in this study:}
851c710
<    %\item By modifying the cooling methodology of the burner rig, the cooling rate was drastically modified;
---
>     \item \rev{By modifying the cooling methodology of the burner rig, the cooling rate was drastically modified;
854,857c713,716
<     \item Local overheating is a direct function of the air gap between the blister and the metallic bond layer. \rev{SEM analysis shows that the overheating is high enough to promote sintering of the TC layer at the top of the blister, while the adherent TC remains unaffected;}
<     %\item This local overheating plays a key role in blister development; 
<     %\item SEM analysis shows that the overheating is high enough to promote sintering of the TC layer at the top of the blister, while the adherent TC remains unaffected;
<     %\item Oxide growth and phase transformation in the BC layer are consistent with homogeneous thermal cycling for similar time at high temperature;
---
>     \item Local overheating is a direct function of the air gap between the blister and the metallic bond layer;
>     \item This local overheating plays a key role in blister development; 
>     \item SEM analysis shows that the overheating is high enough to promote sintering of the TC layer at the top of the blister, while the adherent TC remains unaffected;
>     \item Oxide growth and phase transformation in the BC layer are consistent with homogeneous thermal cycling for similar time at high temperature;
861c720
<     \item Comparisons with standard furnace cycling tests are limited due to data constraints.
---
>     \item Comparisons with standard furnace cycling tests are limited due to data constraints.}.
863c722
< The significant influence of the thermal transient has been clearly demonstrated using the LASDAM technique and should be further strengthened in the FCT analysis. These aspects should be addressed in future publications through a combination of finite element analysis and correlation with experimental temperature measurements. 
---
> \rev{The significant influence of the thermal transient has been clearly demonstrated using the LASDAM technique and should be further strengthened in the FCT analysis}. These aspects should be addressed in future publications through a combination of finite element analysis and correlation with experimental temperature measurements. 
867,868d725
< %Sintering impact is a second order parameter.
< 
869a727
> \section*{References}
874,875c732,951
<  \bibliographystyle{elsarticle-num} 
<  \bibliography{refs,gradbib}
---
>  %\bibliographystyle{elsarticle-num} 
>  %\bibliography{refs,gradbib}
> \begin{thebibliography}{10}
> 	\expandafter\ifx\csname url\endcsname\relax
> 	\def\url#1{\texttt{#1}}\fi
> 	\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
> 	\expandafter\ifx\csname href\endcsname\relax
> 	\def\href#1#2{#2} \def\path#1{#1}\fi
> 	
> 	\bibitem{Evans:2008}
> 	A.~G. Evans, D.~Clarke, C.~Levi, The influence of oxides on the performance of
> 	advanced gas turbines, Journal of the European Ceramic Society 28 (2008)
> 	1405--1419.
> 	
> 	\bibitem{maurel2022coated}
> 	V.~Maurel, M.~Bartsch, M.-H. Vidal-S{\'e}tif, R.~Va{\ss}en, V.~Guipont, Coated
> 	single crystal superalloys: processing, characterization, and modeling of
> 	protective coatings, in: Nickel Base Single Crystals Across Length Scales,
> 	Elsevier, 2022, pp. 283--338.
> 	
> 	\bibitem{Tolpygo:2000}
> 	V.~Tolpygo, D.~Clarke, Surface rumpling of a (ni,pt)al bond coat induced by
> 	cyclic oxidation, Acta Mater. 48 (2000) 3283--3293.
> 	
> 	\bibitem{Tolpygo:2001}
> 	V.~Tolpygo, D.~Clarke, K.~Murphy, Oxidation-induced failure of {EB-PVD} thermal
> 	barrier coatings, Surf. Coat. Technol. 146-147 (2001) 124--131.
> 	
> 	\bibitem{Tolpygo:2004a}
> 	V.~Tolpygo, D.~Clarke, On the rumpling mechanism in nickel-aluminide coatings.
> 	Part I : an experimental assesment., Acta Mater. 52 (2004) 5115--5127.
> 	
> 	\bibitem{Yanar:2006}
> 	N.~Yanar, F.~Pettit, G.~Meier,
> 	\href{http://dx.doi.org/10.1007/s11661-006-0100-4}{Failure characteristics
> 		during cyclic oxidation of yttria stabilized zirconia thermal barrier
> 		coatings deposited via electron beam physical vapor deposition on platinum
> 		aluminide and on nicocraly bond coats with processing modifications for
> 		improved performances}, Metallurgical and Materials Transactions A 37~(5)
> 	(2006) 1563--1580.
> 	
> 	\bibitem{Courcier:2011}
> 	C.~Courcier, V.~Maurel, L.~Remy, S.~Quilici, I.~Rouzou, A.~Phelippeau,
> 	\href{http://www.sciencedirect.com/science/article/B6TVV-51Y57FC-4/2/d26ec16a1de5b850aa59dce80eaa469c}{Interfacial
> 		damage based life model for eb-pvd thermal barrier coating}, Surface and
> 	Coatings Technology 205~(13-14) (2011) 3763 -- 3773.
> 	\newblock \href {https://doi.org/DOI: 10.1016/j.surfcoat.2011.01.008}
> 	{\path{doi:DOI: 10.1016/j.surfcoat.2011.01.008}}.
> 	\newline\urlprefix\url{http://www.sciencedirect.com/science/article/B6TVV-51Y57FC-4/2/d26ec16a1de5b850aa59dce80eaa469c}
> 	
> 	\bibitem{scotson2024characterisation}
> 	D.~Scotson, A.~H. Paksoy, P.~Xiao, Characterisation techniques for
> 	investigating tbc and ebc failure: a review, Frontiers in Ceramics 1 (2024)
> 	1307437.
> 	
> 	\bibitem{Mahfouz:2023}
> 	L.~Mahfouz, B.~Marchand, V.~Guipont, F.~Coudon, V.~Maurel,
> 	\href{https://www.sciencedirect.com/science/article/pii/S2589152923000558}{Driving
> 		forces in thermal barrier coatings blistering}, Materialia 28 (2023) 101728.
> 	\newblock \href {https://doi.org/https://doi.org/10.1016/j.mtla.2023.101728}
> 	{\path{doi:https://doi.org/10.1016/j.mtla.2023.101728}}.
> 	\newline\urlprefix\url{https://www.sciencedirect.com/science/article/pii/S2589152923000558}
> 	
> 	\bibitem{boustie:2007}
> 	M.~Boustie, J.~P. Cuq-Lelandais, C.~Bolis, L.~Berthe, S.~Barradas, M.~Arrigoni,
> 	T.~de~Resseguier, M.~Jeandin,
> 	\href{http://stacks.iop.org/0022-3727/40/i=22/a=036?key=crossref.c6d1d79cc5e14af863b17c7821dcadc5}{Study
> 		of damage phenomena induced by edge effects into materials under laser driven
> 		shocks}, Journal of Physics D: Applied Physics 40~(22) (2007) 7103--7108.
> 	\newblock \href {https://doi.org/10.1088/0022-3727/40/22/036}
> 	{\path{doi:10.1088/0022-3727/40/22/036}}.
> 	\newline\urlprefix\url{http://stacks.iop.org/0022-3727/40/i=22/a=036?key=crossref.c6d1d79cc5e14af863b17c7821dcadc5}
> 	
> 	\bibitem{guipont:2019}
> 	V.~Guipont, G.~Begue, G.~Fabre, V.~Maurel,
> 	\href{http://www.sciencedirect.com/science/article/pii/S0257897219309193}{Buckling
> 		and interface strength analyses of eb-pvd tbc combining laser shock adhesion
> 		test (lasat) to thermal cycling}, Surf. Coat. Technol. under edition~(special
> 	issue 46th ICMCTF) (2019).
> 	\newblock \href
> 	{https://doi.org/https://doi.org/10.1016/j.surfcoat.2019.124938}
> 	{\path{doi:https://doi.org/10.1016/j.surfcoat.2019.124938}}.
> 	\newline\urlprefix\url{http://www.sciencedirect.com/science/article/pii/S0257897219309193}
> 	
> 	\bibitem{levi2012environmental}
> 	C.~G. Levi, J.~W. Hutchinson, M.-H. Vidal-S{\'e}tif, C.~A. Johnson,
> 	Environmental degradation of thermal-barrier coatings by molten deposits, MRS
> 	bulletin 37~(10) (2012) 932--941.
> 	
> 	\bibitem{hutchinson2002delamination}
> 	J.~Hutchinson, A.~Evans, On the delamination of thermal barrier coatings in a
> 	thermal gradient, Surface and Coatings Technology 149~(2-3) (2002) 179--184.
> 	
> 	\bibitem{padture2002}
> 	N.~P. Padture, M.~Gell, E.~H. Jordan, Thermal barrier coatings for gas-turbine
> 	engine applications, Science 296~(5566) (2002) 280--284.
> 	
> 	\bibitem{EvansHE:2011}
> 	H.~E. Evans,
> 	\href{http://www.sciencedirect.com/science/article/pii/S0257897211005949}{Oxidation
> 		failure of tbc systems: An assessment of mechanisms}, Surface and Coatings
> 	Technology 206~(7) (2011) 1512 -- 1521.
> 	\newblock \href {https://doi.org/10.1016/j.surfcoat.2011.05.053}
> 	{\path{doi:10.1016/j.surfcoat.2011.05.053}}.
> 	\newline\urlprefix\url{http://www.sciencedirect.com/science/article/pii/S0257897211005949}
> 	
> 	\bibitem{li2017correlation}
> 	C.-J. Li, H.~Dong, H.~Ding, G.-J. Yang, C.-X. Li, The correlation of the tbc
> 	lifetimes in burner cycling test with thermal gradient and furnace isothermal
> 	cycling test by tgo effects, Journal of Thermal Spray Technology 26 (2017)
> 	378--387.
> 	
> 	\bibitem{vassen2000}
> 	R.~Va{\ss}en, X.~Cao, F.~Tietz, D.~Basu, D.~St{\"o}ver, Zirconates as new
> 	materials for thermal barrier coatings, Journal of the American Ceramic
> 	Society 83~(8) (2000) 2023--2028.
> 	
> 	\bibitem{kim2021method}
> 	D.~Kim, K.~Park, K.~Kim, C.-S. Seok, J.~Lee, K.~Kim, A method for predicting
> 	the delamination life of thermal barrier coatings under thermal gradient
> 	mechanical fatigue condition considering degradation characteristics,
> 	International Journal of Fatigue 151 (2021) 106402.
> 	
> 	\bibitem{wu2019laser}
> 	Y.~Wu, P.-f. Hsu, Y.~Wang, M.~H. McCay, D.~E. Croy, D.~Moreno, L.~He, C.~Wang,
> 	H.~Zhang, Laser thermal gradient testing and fracture mechanics study of a
> 	thermal barrier coating, Journal of Thermal Spray Technology 28 (2019)
> 	1239--1251.
> 	
> 	\bibitem{qian1998effects}
> 	G.~Qian, T.~Nakamura, C.~Berndt, Effects of thermal gradient and residual
> 	stresses on thermal barrier coating fracture, Mechanics of Materials 27~(2)
> 	(1998) 91--110.
> 	
> 	\bibitem{sniezewski2009thermal}
> 	J.~Sniezewski, V.~Vidal, P.~Lours, Y.~Le~Maoult, Thermal barrier coatings
> 	adherence and spallation: Interfacial indentation resistance and cyclic
> 	oxidation behaviour under thermal gradient, Surface and Coatings Technology
> 	204~(6-7) (2009) 807--811.
> 	
> 	\bibitem{jiang2019numerical}
> 	J.~Jiang, L.~Jiang, Z.~Cai, W.~Wang, X.~Zhao, Y.~Liu, Z.~Cao, Numerical stress
> 	analysis of the tbc-film cooling system under operating conditions
> 	considering the effects of thermal gradient and tgo growth, Surface and
> 	Coatings Technology 357 (2019) 433--444.
> 	
> 	\bibitem{benoist2004microstructure}
> 	J.~Benoist, K.~Badawi, A.~Mali{\'e}, C.~Ramade, Microstructure of pt-modified
> 	aluminide coatings on ni-based superalloys, Surface and Coatings Technology
> 	182~(1) (2004) 14--23.
> 	
> 	\bibitem{audigie2019high}
> 	P.~Audigi{\'e}, A.~R.-V. Put, A.~Mali{\'e}, C.~Thouron, D.~Monceau,
> 	High-temperature cyclic oxidation of pt-rich
> 	$\gamma$-$\gamma$’bond-coatings. part ii: Effect of pt and al on tbc system
> 	lifetime, Corrosion Science 150 (2019) 1--8.
> 	
> 	\bibitem{sapardanis:2016}
> 	H.~Sapardanis, V.~Maurel, A.~K{\"o}ster, S.~Duvinage, F.~Borit, V.~Guipont,
> 	Influence of macroscopic shear loading on the growth of an interfacial crack
> 	initiated from a ceramic blister processed by laser shock, Surface and
> 	Coatings Technology 291 (2016) 430--443.
> 	
> 	\bibitem{sapardanis:2017}
> 	H.~Sapardanis, V.~Guipont, F.~Borit, A.~Debray, A.~K{\"o}ster, V.~Maurel, Study
> 	of the interface strength and residual stresses within plasma sprayed alumina
> 	coatings involving lasat (laser shock adhesion test), in: International
> 	thermal spray conference 2017, DVS Berichte, 2017, pp. 315--321.
> 	
> 	\bibitem{maurel:2019}
> 	V.~Maurel, V.~Guipont, M.~Theveneau, B.~Marchand, F.~Coudon, Thermal cycling
> 	damage monitoring of thermal barrier coating assisted with lasat (laser shock
> 	adhesion test), Surface and Coatings Technology 380 (2019) 125048.
> 	
> 	\bibitem{Vassen2020}
> 	R.~Vaßen, D.~Mack, M.~Tandler, Y.~Sohn, D.~Sebold, O.~Guillon, Unique
> 	performance of thermal barrier coatings made of yttria stabilized zirconia at
> 	extreme temperatures (> 1500°c), Journal of the American Ceramic Society 104
> 	(09 2020).
> 	\newblock \href {https://doi.org/10.1111/jace.17452}
> 	{\path{doi:10.1111/jace.17452}}.
> 	
> 	\bibitem{soulignac2014prevision}
> 	R.~Soulignac, Pr{\'e}vision de la dur{\'e}e de vie {\`a} l’{\'e}caillage des
> 	barri{\`e}res thermiques (in french), Ph.D. thesis, Ecole Nationale
> 	Sup{\'e}rieure des Mines de Paris (2014).
> 	
> 	\bibitem{ImageJ:2024}
> 	ImageJ, Image processing and analysis in java, v2.15.1,
> 	https://imagej.net/software/fiji/ (2024).
> 	
> 	\bibitem{Maurel:2012b}
> 	V.~Maurel, L.~Helfen, F.~N'Guyen, A.~Koster, M.~D. Michiel, T.~Baumbach,
> 	T.~Morgeneyer,
> 	\href{http://www.sciencedirect.com/science/article/pii/S135964621100769X}{Three-dimensional
> 		investigation of thermal barrier coatings by synchrotron-radiation computed
> 		laminography}, Scripta Materialia 66~(7) (2012) 471 -- 474.
> 	\newblock \href {https://doi.org/10.1016/j.scriptamat.2011.12.021}
> 	{\path{doi:10.1016/j.scriptamat.2011.12.021}}.
> 	\newline\urlprefix\url{http://www.sciencedirect.com/science/article/pii/S135964621100769X}
> 	
> 	\bibitem{Maurel:2012f}
> 	V.~Maurel, R.~Soulignac, L.~Helfen, T.~Morgeneyer, A.~Koster, L.~Remy,
> 	Three-dimensional damage evolution measurement in ebpvd tbc using synchrotron
> 	laminography, Oxidat. of Metals {79}~({3-4, SI}) ({2013}) {313--323}.
> 	
> 	\bibitem{mcdonald:2010}
> 	J.~P. McDonald, M.~Thouless, S.~M. Yalisove, Mechanics analysis of femtosecond
> 	laser-induced blisters produced in thermally grown oxide on si(100), Journal
> 	of Materials Research 25~(6) (2010) 1087?1095.
> 	\newblock \href {https://doi.org/10.1557/JMR.2010.0146}
> 	{\path{doi:10.1557/JMR.2010.0146}}.
> 	
> 	\bibitem{vassen2009}
> 	R.~Va{\ss}en, S.~Giesen, D.~St{\"o}ver, Lifetime of plasma-sprayed thermal
> 	barrier coatings: Comparison of numerical and experimental results, Journal
> 	of Thermal Spray Technology 18~(5-6) (2009) 835--845.
> 	
> \end{thebibliography}
> 

